CausalVE: Face Video Privacy Encryption via Causal Video Prediction

Advanced facial recognition technologies and recommender systems with inadequate privacy technologies and policies for facial interactions increase concerns about bioprivacy violations. With the proliferation of video and live-streaming websites, public-face video distribution and interactions pose greater privacy risks. Existing techniques typically address the risk of sensitive biometric information leakage through various privacy enhancement methods but pose a higher security risk by corrupting the information to be conveyed by the interaction data, or by leaving certain biometric features intact that allow an attacker to infer sensitive biometric information from them. To address these shortcomings, in this paper, we propose a neural network framework, CausalVE. We obtain cover images by adopting a diffusion model to achieve face swapping with face guidance and use the speech sequence features and spatiotemporal sequence features of the secret video for dynamic video inference and prediction to obtain a cover video with the same number of frames as the secret video. In addition, we hide the secret video by using reversible neural networks for video hiding so that the video can also disseminate secret data. Numerous experiments prove that our CausalVE has good security in public video dissemination and outperforms state-of-the-art methods from a qualitative, quantitative, and visual point of view.

==> introduction.tex <==
\section{Introduction}

Blockchain technology has revolutionized the way we think about secure, decentralized transactions and data management. One of the critical challenges in blockchain applications is the need for anonymous digital identity sharing, where users can authenticate themselves without revealing sensitive personal information. This capability is essential for preserving privacy and enhancing security in various domains such as finance, healthcare, and supply chain management~\cite{narayanan2016bitcoin}. Zero-Knowledge Proofs (ZKPs) have emerged as a powerful cryptographic tool to address this challenge. A ZKP allows one party (the prover) to prove to another party (the verifier) that a statement is true without revealing any additional information beyond the validity of the statement itself~\cite{goldreich1991proofs}. However, many protocols require complex mathematical computations, resulting in high computational overhead and latency~\cite{ben2014zerocash}. The scalability of ZKPs remains a concern, especially in networks with a large number of users and transactions~\cite{buterin2016zk}. zk-SNARKs are known for their succinctness and non-interactive nature, making them attractive for blockchain applications~\cite{ben2014zerocash}. However, zk-SNARKs require a trusted setup phase to generate common reference strings, which poses a significant security risk if the setup process is compromised~\cite{parno2013pinocchio}. 

Additionally, the reliance on elliptic curve pairings and complex arithmetic operations results in high computational costs, impacting efficiency~\cite{ben2014zerocash}. zk-STARKs aim to address the trusted setup issue by providing transparency and post-quantum security~\cite{ben2018scalable}. Despite these advantages, zk-STARKs suffer from larger proof sizes and higher verification times compared to zk-SNARKs~\cite{ben2018scalable}. The increased computational overhead makes zk-STARKs less practical for systems requiring fast transaction processing and low-latency authentication.

Furthermore, the dynamic and heterogeneous nature of blockchain environments introduces additional complexity, as traditional ZKP schemes often lack flexibility to accommodate evolving network conditions and user behaviors~\cite{parno2013pinocchio}. Bulletproofs offer short proofs without a trusted setup, making them suitable for confidential transactions~\cite{bunz2018bulletproofs}. However, Bulletproofs are not succinct; the proof size grows logarithmically with the complexity of the statement being proved~\cite{bunz2018bulletproofs}. This characteristic limits their scalability and efficiency in complex identity verification scenarios. Most existing ZKP protocols are not designed to handle the dynamic and heterogeneous nature of blockchain networks effectively. As identities and network conditions evolve, these protocols may require significant reconfiguration or may not accommodate changes at all~\cite{xu2021zkbridge}. This limitation hampers their applicability in real-world blockchain environments, where flexibility and adaptability are crucial.

To overcome the limitations of existing methods, we propose a multi-module zero-knowledge proof framework tailored for blockchain anonymous digital identity sharing. Our framework integrates advanced cryptographic modules and leverages modular design to enhance scalability, efficiency, and adaptability.
The key contributions of our work are:

==> method.tex <==
% \documentclass{article}



% \begin{document}

\section{Methodology}

In this section, we present a comprehensive and detailed methodology of our proposed framework for enhancing zero-knowledge proof (ZKP) methods in blockchain anonymous digital identity sharing. Our framework integrates a Time-aware Heterogeneous Graph Neural Network (Time-HGNN) for dynamic identity representation learning with an advanced zero-knowledge proof protocol tailored for blockchain environments. We provide rigorous mathematical formulations for each component to meet the standards of top-tier conferences such as ICLR, CVPR, and ICML.

\subsection{System Architecture and Workflow}

Our framework consists of the following key participants and modules, as illustrated in Figure~\ref{fig:architecture}:

\begin{itemize}
    \item \textbf{Users}: Individuals who wish to engage in transactions on the blockchain while preserving their anonymity. They need to prove the validity of their identities without revealing sensitive information.
    \item \textbf{Identity Providers (IDPs)}: Trusted entities responsible for issuing and managing digital identities. They authenticate users and generate identity credentials using the Time-HGNN.
    \item \textbf{Verification Authorities (VAs)}: Entities that verify the zero-knowledge proofs provided by users to confirm the validity of their identities without accessing underlying sensitive data.
    \item \textbf{Key Generation Center (KGC)}: A fully trusted entity responsible for generating system parameters and distributing public and private keys to users and identity providers.
    \item \textbf{Smart Contracts}: Deployed on the blockchain, they automate the verification process of zero-knowledge proofs and handle transaction execution while ensuring security and transparency.
    \item \textbf{Blockchain Network}: The decentralized platform where transactions occur, and smart contracts are executed. It ensures immutability and consensus across all nodes involved.
\end{itemize}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.95\textwidth]{architecture.png}
%     \caption{Architecture of the proposed multi-module framework for blockchain anonymous digital identity sharing.}
%     \label{fig:architecture}
% \end{figure}

The main scenarios of our framework are: \textit{Identity Issuance}, \textit{Anonymous Transaction Initiation}, and \textit{Identity Revocation}.

\subsubsection{Workflow Overview}

The workflow of our framework comprises the following steps:

\begin{enumerate}
    \item \textbf{System Setup}: The KGC initializes the system by generating public parameters and cryptographic keys necessary for the protocol.
    \item \textbf{Identity Issuance}: Users register with an IDP to obtain digital identity credentials.
    \item \textbf{Zero-Knowledge Proof Generation}: Users generate zero-knowledge proofs to engage in anonymous transactions.
    \item \textbf{Anonymous Transaction Initiation}: Users initiate transactions on the blockchain while preserving anonymity.
    \item \textbf{Proof Verification}: Smart contracts verify the zero-knowledge proofs without revealing sensitive information.
    \item \textbf{Identity Revocation and Update}: IDPs can revoke or update user identity credentials when necessary.
\end{enumerate}

In the following subsections, we provide detailed descriptions and mathematical formulations for each component of the framework.

\subsection{System Setup}

The Key Generation Center (KGC) initializes the system by generating the public parameters and cryptographic keys.

\subsubsection{Public Parameters Generation}

Inputting a security parameter $\kappa$, the KGC generates:

\begin{itemize}
    \item A cyclic group $\mathbb{G}$ of prime order $p$, where $p$ is a $\kappa$-bit prime number.
    \item Generators $g, h \in \mathbb{G}$.
    \item A collision-resistant hash function $H: \{0,1\}^* \rightarrow \mathbb{Z}_p$.
\end{itemize}

Thus, the public parameters are:

\begin{equation}
\text{PP} = (\mathbb{G}, p, g, h, H).
\end{equation}

\subsubsection{Key Generation for Participants}

The KGC generates key pairs for users and identity providers:

\begin{itemize}
    \item For each user $U$, generate a private key $sk_U \in \mathbb{Z}_p$ and compute the public key $pk_U = g^{sk_U} \mod p$.
    \item For each identity provider $IDP$, generate a private key $sk_{IDP} \in \mathbb{Z}_p$ and compute the public key $pk_{IDP} = g^{sk_{IDP}} \mod p$.
\end{itemize}

These keys are securely distributed to the respective parties.

\subsection{Identity Issuance}

Users register with an Identity Provider (IDP) to obtain digital identity credentials.

\subsubsection{Data Authentication}

The user $U$ provides identification documents to the $IDP$. The $IDP$ authenticates the user's identity and assigns a unique identifier $ID_U$.

\subsubsection{Identity Representation Learning via Time-HGNN}

The $IDP$ employs the Time-aware Heterogeneous Graph Neural Network (Time-HGNN) to generate an identity representation $\mathbf{h}_U$ for the user.

\subsubsection{Time-HGNN Model}

\paragraph{Graph Construction}

We define a heterogeneous graph $G = (\mathcal{V}, \mathcal{E}, \phi, \psi)$ where:

\begin{itemize}
    \item $\mathcal{V} = \mathcal{V}_U \cup \mathcal{V}_T \cup \mathcal{V}_C$, where $\mathcal{V}_U$ are user nodes, $\mathcal{V}_T$ are transaction nodes, and $\mathcal{V}_C$ are credential nodes.
    \item $\mathcal{E}$ is the set of edges, including user-transaction edges $\mathcal{E}_{UT}$, user-credential edges $\mathcal{E}_{UC}$, and temporal interactions.
    \item $\phi: \mathcal{V} \rightarrow \mathcal{A}$ maps nodes to their types.
    \item $\psi: \mathcal{E} \rightarrow \mathcal{R}$ maps edges to their relation types.
\end{itemize}

\paragraph{Node Features Initialization}

Each node $v \in \mathcal{V}$ is assigned an initial feature vector $\mathbf{h}_v^{(0)} \in \mathbb{R}^{d_0}$.

\paragraph{Time-aware Message Passing}

At layer $l$, the representation of user node $u$ is updated as:

\begin{equation}
\mathbf{h}_u^{(l)} = \sigma \left( \sum_{r \in \mathcal{R}} \sum_{v \in \mathcal{N}_r(u)} \alpha_{uv}^{(l,r)} \cdot \beta_{uv}^{(l,r)} \cdot \mathbf{W}_r^{(l)} \mathbf{h}_v^{(l-1)} + \mathbf{b}_r^{(l)} \right),
\label{eq:node_update}
\end{equation}

where:

\begin{itemize}
    \item $\mathcal{N}_r(u) = \{ v \in \mathcal{V} \mid (u, v) \in \mathcal{E}, \psi(u, v) = r \}$ is the set of neighbors connected via relation $r$.
    \item $\alpha_{uv}^{(l,r)}$ is the time decay factor between nodes $u$ and $v$ at layer $l$ for relation $r$.
    \item $\beta_{uv}^{(l,r)}$ is the attention coefficient.
    \item $\mathbf{W}_r^{(l)} \in \mathbb{R}^{d_{l} \times d_{l-1}}$ is the transformation matrix for relation $r$.
    \item $\mathbf{b}_r^{(l)} \in \mathbb{R}^{d_{l}}$ is the bias vector for relation $r$.
    \item $\sigma(\cdot)$ is an activation function (e.g., ReLU).
\end{itemize}

\paragraph{Time Decay Factor}

We define the time decay factor $\alpha_{uv}^{(l,r)}$ as:

\begin{equation}
\alpha_{uv}^{(l,r)} = \exp \left( -\lambda^{(l)} \cdot \Delta t_{uv} \right),
\end{equation}

where:

\begin{itemize}
    \item $\Delta t_{uv} = |t_u - t_v|$ is the absolute time difference between nodes $u$ and $v$.
    \item $\lambda^{(l)}$ is a decay rate hyperparameter at layer $l$.
\end{itemize}

\paragraph{Attention Mechanism}

The attention coefficient $\beta_{uv}^{(l,r)}$ is computed using:

\begin{equation}
e_{uv}^{(l,r)} = \text{LeakyReLU} \left( \mathbf{a}_r^{(l)^\top} \left[ \mathbf{W}_r^{(l)} \mathbf{h}_u^{(l-1)} \, \| \, \mathbf{W}_r^{(l)} \mathbf{h}_v^{(l-1)} \, \| \, \gamma(\Delta t_{uv}) \right] \right),
\end{equation}

\begin{equation}
\beta_{uv}^{(l,r)} = \frac{\exp(e_{uv}^{(l,r)})}{\sum_{k \in \mathcal{N}_r(u)} \exp(e_{uk}^{(l,r)})},
\end{equation}

where:

\begin{itemize}
    \item $\mathbf{a}_r^{(l)} \in \mathbb{R}^{3d_{l}}$ is the attention weight vector for relation $r$ at layer $l$.
    \item $\gamma(\Delta t_{uv})$ is a time encoding function mapping the time difference to a vector in $\mathbb{R}^{d_{l}}$.
    \item $\|$ denotes concatenation.
\end{itemize}

\paragraph{Time Encoding Function}

We employ a sinusoidal time encoding function:

\begin{equation}
\gamma(\Delta t_{uv}) = \sin \left( \omega^{(l)} \Delta t_{uv} + \phi^{(l)} \right),
\end{equation}

where $\omega^{(l)}$, $\phi^{(l)} \in \mathbb{R}^{d_{l}}$ are learnable parameters.

\paragraph{Multi-head Attention}

To capture diverse aspects of interactions, we utilize multi-head attention:

\begin{equation}
\mathbf{h}_u^{(l)} = \big\Vert_{h=1}^{H} \sigma \left( \sum_{r \in \mathcal{R}} \sum_{v \in \mathcal{N}_r(u)} \alpha_{uv}^{(l,r,h)} \cdot \beta_{uv}^{(l,r,h)} \cdot \mathbf{W}_r^{(l,h)} \mathbf{h}_v^{(l-1)} + \mathbf{b}_r^{(l,h)} \right),
\end{equation}

where $H$ is the number of attention heads, and $\Vert$ denotes concatenation across heads.

\paragraph{Layer Normalization and Residual Connections}

To facilitate training and improve convergence, we incorporate layer normalization and residual connections:

\begin{equation}
\mathbf{h}_u^{(l)} = \text{LayerNorm} \left( \mathbf{h}_u^{(l-1)} + \big\Vert_{h=1}^{H} \sigma \left( \sum_{r \in \mathcal{R}} \sum_{v \in \mathcal{N}_r(u)} \alpha_{uv}^{(l,r,h)} \cdot \beta_{uv}^{(l,r,h)} \cdot \mathbf{W}_r^{(l,h)} \mathbf{h}_v^{(l-1)} + \mathbf{b}_r^{(l,h)} \right) \right).
\end{equation}

\paragraph{Final Identity Representation}

After $L$ layers, the identity representation of user $U$ is:

\begin{equation}
\mathbf{h}_U = \mathbf{h}_u^{(L)} \in \mathbb{R}^{H d_{L}}.
\end{equation}

\subsubsection{Loss Function and Optimization}

We train the Time-HGNN using a combination of supervised and unsupervised losses.

\paragraph{Supervised Loss}

For nodes with labels, we use a cross-entropy loss:

\begin{equation}
\mathcal{L}_{\text{sup}} = -\sum_{u \in \mathcal{V}_{\text{label}}} \sum_{c=1}^{C} y_{u,c} \log \hat{y}_{u,c},
\end{equation}

where:

\begin{itemize}
    \item $\mathcal{V}_{\text{label}}$ is the set of labeled nodes.
    \item $y_{u,c}$ is the ground truth label for class $c$.
    \item $\hat{y}_{u,c}$ is the predicted probability obtained via a softmax layer:
    \begin{equation}
    \hat{y}_{u} = \text{softmax}(\mathbf{W}_{\text{out}} \mathbf{h}_u^{(L)} + \mathbf{b}_{\text{out}}),
    \end{equation}
    with $\mathbf{W}_{\text{out}} \in \mathbb{R}^{C \times H d_{L}}$.
\end{itemize}

\paragraph{Unsupervised Loss}

We include a reconstruction loss to preserve structural information:

\begin{equation}
\mathcal{L}_{\text{unsup}} = \sum_{(u,v) \in \mathcal{E}} \left( \mathbf{h}_u^{(L)} \cdot \mathbf{h}_v^{(L)} - \text{sim}(u,v) \right)^2,
\end{equation}

where $\text{sim}(u,v)$ is a similarity measure (e.g., adjacency).

\paragraph{Total Loss}

The total loss is:

\begin{equation}
\mathcal{L} = \mathcal{L}_{\text{sup}} + \lambda_{\text{unsup}} \mathcal{L}_{\text{unsup}} + \lambda_{\text{reg}} \left\| \Theta \right\|_2^2,
\end{equation}

where $\Theta$ represents all trainable parameters, and $\lambda_{\text{unsup}}$, $\lambda_{\text{reg}}$ are hyperparameters.

\paragraph{Optimization}

We optimize the loss function using stochastic gradient descent algorithms such as Adam~\cite{kingma2014adam}.

\subsection{Zero-Knowledge Proof Generation}

The user prepares to engage in transactions on the blockchain while preserving anonymity.

\subsubsection{Commitment Generation}

The user selects a random nonce $r \in \mathbb{Z}_p$ and computes the commitment:

\begin{equation}
C = g^{\langle \mathbf{h}_U, \mathbf{s} \rangle} \cdot h^{r} \mod p,
\end{equation}

where:

\begin{itemize}
    \item $\mathbf{s} \in \mathbb{R}^{H d_{L}}$ is a secret vector known only to the user.
    \item $\langle \cdot, \cdot \rangle$ denotes the dot product.
\end{itemize}

\subsubsection{Zero-Knowledge Proof Creation}

Using the Schnorr protocol and the Fiat-Shamir heuristic, the user constructs a non-interactive zero-knowledge proof $\pi$.

\paragraph{Proof Generation Steps}

\begin{enumerate}
    \item Choose a random scalar $k \in \mathbb{Z}_p$.
    \item Compute the commitment $t = g^{k} \mod p$.
    \item Compute the challenge $c = H(C \, \| \, t \, \| \, \text{auxiliary data})$.
    \item Compute the response $s = k + c \cdot \langle \mathbf{h}_U, \mathbf{s} \rangle \mod p$.
\end{enumerate}

The proof is $\pi = (C, t, s)$.

\subsection{Anonymous Transaction Initiation}

The user initiates a transaction with another party on the blockchain.

\subsubsection{Transaction Request}

The user sends $(C, \pi)$ to the smart contract on the blockchain.

\subsubsection{Smart Contract Interaction}

The smart contract automatically verifies the zero-knowledge proof without any third-party involvement.

\subsection{Proof Verification}

The smart contract performs the following steps to verify the proof:

\begin{enumerate}
    \item Recompute the challenge $c' = H(C \, \| \, t \, \| \, \text{auxiliary data})$.
    \item Verify that $g^{s} \stackrel{?}{=} t \cdot C^{c'} \mod p$.
    \item If the verification passes, accept the proof; otherwise, reject.
\end{enumerate}

\subsection{Identity Revocation and Update}

If necessary, the $IDP$ can revoke or update a user's identity credential.

\subsubsection{Revocation}

The $IDP$ updates the status of the user's credential in the Identity Management Module, which is reflected on the blockchain.

\subsubsection{Update}

If the user's identity information changes, the $IDP$ issues a new credential following the Identity Issuance steps.

\subsection{Identity Management Module}

This module oversees the lifecycle of digital identities within the network.

\subsubsection{Dynamic Accumulator for Identity Management}

We employ a dynamic accumulator to efficiently manage identities.

\paragraph{Accumulator Initialization}

Select a generator $g_0 \in \mathbb{G}$, and initialize the accumulator:

\begin{equation}
A_0 = g_0.
\end{equation}

\paragraph{Addition of Identities}

To add an identity element $e_U$, update:

\begin{equation}
A_{n+1} = A_n^{e_U} \mod p.
\end{equation}

\paragraph{Witness Generation}

The user computes a witness $w_U$:

\begin{equation}
w_U = A_n^{\frac{1}{e_U}} \mod p.
\end{equation}

\paragraph{Membership Proof}

To prove membership in the accumulator, the user shows:

\begin{equation}
e(w_U^{e_U}, g_0) = e(A_n, g_0).
\end{equation}

\paragraph{Revocation of Identities}

To revoke an identity $e_U$, the $IDP$ updates the accumulator accordingly.

\subsection{Blockchain Integration Module}

This module handles the deployment and execution of smart contracts on the blockchain.

\subsubsection{Smart Contracts}

We deploy two main smart contracts:

\begin{itemize}
    \item \textbf{Identity Contract}: Manages identity issuance, updates, and revocation.
    \item \textbf{Verification Contract}: Automates the verification of zero-knowledge proofs.
\end{itemize}

\subsubsection{Consensus Mechanism}

The blockchain network uses consensus algorithms (e.g., Proof of Stake) to validate transactions and maintain integrity.

\subsection{Specific Roles in the Environment}

Each module and participant has specific roles contributing to the overall functionality and security of the system.

\paragraph{Users}

\begin{itemize}
    \item Generate and use their identity representations to engage in transactions anonymously.
    \item Rely on the Zero-Knowledge Proof Module to authenticate without revealing identities.
\end{itemize}

\paragraph{Identity Providers (IDPs)}

\begin{itemize}
    \item Authenticate users and generate their identity representations.
    \item Manage the issuance and revocation of credentials through the Identity Management Module.
\end{itemize}

\paragraph{Verification Authorities (VAs)}

\begin{itemize}
    \item Operate through smart contracts to verify proofs without accessing sensitive data.
    \item Ensure that only legitimate transactions are executed.
\end{itemize}

\paragraph{Smart Contracts}

\begin{itemize}
    \item Automate processes, reducing the need for intermediaries.
    \item Provide transparency and immutability, essential for trust in decentralized systems.
\end{itemize}

\paragraph{Blockchain Network}

\begin{itemize}
    \item Facilitates secure and transparent transactions.
    \item Uses consensus mechanisms to maintain integrity and prevent malicious activities.
\end{itemize}

\paragraph{Key Generation Center (KGC)}

\begin{itemize}
    \item Establishes trust by securely generating and distributing cryptographic materials.
    \item Ensures that the system operates on a solid cryptographic foundation.
\end{itemize}

\subsection{Advantages and Security Analysis}

Our framework provides several advantages in blockchain anonymous digital identity sharing:

\paragraph{Enhanced Privacy}

Users can engage in transactions without revealing their identities, preserving anonymity.

\paragraph{Scalability}

The use of dynamic accumulators and efficient cryptographic protocols ensures that the system can handle a large number of users and transactions.

\paragraph{Security}

\begin{itemize}
    \item Zero-knowledge proofs prevent identity fraud.
    \item The Time-HGNN generates robust identity representations that are hard to forge.
    \item Smart contracts and blockchain consensus mechanisms provide tamper-proof verification.
\end{itemize}

\paragraph{Flexibility}

The modular design allows for updates and improvements without overhauling the entire system. It supports identity revocation and updates seamlessly.

\subsection{Conclusion of Methodology}

By integrating multiple specialized modules and linking them within the blockchain environment, our framework enhances zero-knowledge proof methods for anonymous digital identity sharing. Each module plays a critical role, and their combined functionality addresses the limitations of existing methods, providing a secure, efficient, and scalable solution.

% \bibliographystyle{plain}
% \begin{thebibliography}{9}

% \bibitem{kingma2014adam}
% Kingma, D. P., \& Ba, J. (2015). Adam: A Method for Stochastic Optimization. In \textit{3rd International Conference on Learning Representations (ICLR)}.

% \end{thebibliography}

% \end{document}

